How to Measure Human-AI Prediction Accuracy in Explainable AI Systems

Assessing an AI system's behavior-particularly in Explainable AI Systems-is sometimes done empirically, by measuring people's abilities to predict the agent's next move-but how to perform such measurements? In empirical studies with humans, an obvious approach is to frame the task as binary (i.e., prediction is either right or wrong), but this does not scale. As output spaces increase, so do floor effects, because the ratio of right answers to wrong answers quickly becomes very small. The crux of the problem is that the binary framing is failing to capture the nuances of the different degrees of "wrongness." To address this, we begin by proposing three mathematical bases upon which to measure "partial wrongness." We then uses these bases to perform two analyses on sequential decision-making domains: the first is an in-lab study with 86 participants on a size-36 action space; the second is a re-analysis of a prior study on a size-4 action space. Other researchers adopting our operationalization of the prediction task and analysis methodology will improve the rigor of user studies conducted with that task, which is particularly important when the domain features a large output space.

==> documentBody/leftovers.tex <==
\subsubsection{\underline{A}verage of product of counts and \underline{V}alue losses\draftStatus{D1.0}
}
This strategy is essentially taking a weighted average of participant predictions, using the value as the weight.
The inner sum is simply counting the number of participants who guessed a particular action, while the outer sum combines counts from all actions.
\begin{equation}
AV = \biggl(\sum_{a\in A} \Bigl(\sum_{i=1\ldots|P|} (a == a_i)\Bigr)*V(a)\biggr)/|P|
\label{eqnLVS}
\end{equation}

\subsubsection{\underline{A}verage of product of counts and \underline{R}ank losses\draftStatus{D1.0}
}
Similarly to the last strategy, we use a weighted average, but use the \emph{rank} to weight instead of the value. %JED@TJB: here we mean weight as in to assign weight
\begin{equation}
AR = \biggl(\sum_{a\in A} \Bigl(\sum_{i=1\ldots|P|} (a == a_i)\Bigr)*R(a)\biggr)/|P|\label{eqnAR}
\end{equation}

\hrule



\boldify{However, diverse people do many different tasks in different ways [cite gendermag findings, anything else we got].}

AI assessment is challenging for people to do:  it is a broad problem-solving task, with many possible approaches to performing the task.
As such, we should expect diverse individuals to conduct assessment in various ways.
Thus, solving the eXplainable AI (XAI) problem will require a variety of affordances in terms of explanations and processes for consuming explanation.
While many researchers have proposed a variety of explanations (e.g.,~\cite{arya2019one, mueller2019explanation,  cheng2019explaining}), and some have proposed processes (e.g., ~\cite{Schindler-2003-219, dodgej2021aarai}), the justification for the efficacy of these techniques usually relies on \emph{averaging} all the studied users.
As a result of relying on such averaging, researchers may be missing important effects pertaining to \emph{which techniques} are effective for \emph{which users}.

\boldify{At first, this can lead to one population being under-served by a dominant technique [pre-Gendermag stuff].}

One intellectual tool that has been used to understand the diversity of human problem-solving with technology is the GenderMag method~\cite{burnett2016gendermag-jrnl}.
GenderMag and its components have been used to detect ``inclusivity bugs'' in how technology supports diverse users in a variety of domains, often pointing the way toward fixes (e.g.,~\cite{chatterjee2022inclusivity,letaw2021changing, cunningham2016supporting,  gralha2019genderMagExperiment, guizani2022debug,hilderbrand2020genderMagTalesTrenches, kanij2022genderMagSEjobs, padala2020gender, shekhar2018genderMagLearningSystem}).
Of particular relevance to this paper, some of these investigations have been in AI-based domains, such as: AI-based office productivity products, ML tools for ML practitioners, telerobotics, and search tools~\cite{anderson-diversity-2022, burnett2016finding-chi, showkat2018genderMagTelerobotics,vorvoreanu2019gender}.
This paper leverages cognitive styles, one of the GenderMag components, in our investigation.

\boldify{Although people are considering different demographic information for human-AI information, how do we know that we are selecting/measuring the correct demographics? Other than Anderson et al (under review) few people are studying diversity \textit{of thought} to determine which XAI techniques might be preferred by users with diverse cognitive styles}

In the context of human-AI interaction, researchers sometimes disaggregate their data, considering not just ``the user'' but different categories of users. 
Some examples include analyzing results through the lens of user demographics, such as age~\cite{gillath2021attachment,shahid2014child,martinez2018age}, cultural background~\cite{shahid2014child,rau2009effects}, and gender~\cite{de2015sharing,van2021effect,derrick2014affective}.
However, in the subarea of XAI, few researchers have disaggregated.
One exception is work by Anderson et al.~\cite{anderson-diversity-2022}, who used disaggregation to find inclusivity insights about participants' user experience when Amershi et al.'s~\cite{amershi2019guidelines} 18 guidelines for human-AI interaction were violated or applied.
Another is a study by Dodge, et al.~\cite{dodge-fairness-2019} which found that a large minority of participants felt that it was acceptable to use race features for AI-powered decisions.
Those authors state, \emph{``...the consideration of this individual factor (race position) `de-noised' the data.''}~\cite{dodge-fairness-2019}.
Another more recent example is a study by Riefle et al.~\cite{riefle2022influence} which studied how people with ``rational'' vs. ``intuitive'' cognitive styles approached explanation consumption.



\boldify{This work aims to begin to understand how XAI tasks and techniques affect people with differing information processing styles, using a large scale qualitative study}

Similar to Anderson et al.~\cite{anderson-diversity-2022}'s findings about users' experiences (e.g., feeling in control) while interacting with AI-powered technologies, we believe that disaggregating participants' behavioral data by their information processing style can help uncover diverse processes that users take while trying to understand which moves an intelligent agent will take and why. 
% \FIXME{AAA@MMB: Based on our dicussion this morning, here's a couple ``competitors'' to information processing style:\\
% Affinity for Technology Interaction (ATI)~\cite{franke2019personal}\\
% Need for Cognition~\cite{cohen1955experimental,li2006role,srivastava2010online}}
%We believe, similar to Anderson et al.~\cite{anderson-diversity-2022}, that disaggregating by participants' diversity \textit{of thought} can cut across varying demographic traits to enable the research community to begin understanding how XAI tasks and techniques affect people with diverse cognitive styles, using a large scale qualitative study.



\boldify{During our study, we administered the GenderMag survey so that we might know participants cognitive styles to try to tie it to behavioral observations.
Here are those data}

Before beginning the tutorial, each participant\footnote{One participant did not complete the survey, so we have excluded that participant from relevant analyses.} completed the GenderMag survey~\cite{anderson-diversity-2022,guizani2022debug}.
% \FIXED{MMB: when this paper is accepted, replace with a cite to our hopefully-accepted-by-then book chapter about the survey, which will be a better ref for this (Hamid et al. 2023).}
Our goal in administering this survey was to connect our observations about participant behavior and task performance to this important demographic data.


\FIXME{\boldify{We mucked around in the source to make this study possible, and added some tasks, which are...}

The three tasks that participants went through, using onscreen dialogues\footnote{See Supplemental Materials.}, were:
Comparison (also known as A vs B), Ranking, and Prediction.
Each participant used a different combination of the three explanations for each task, totaling eight treatment combinations, chosen so that each participant would see each individual explanation at least once during the study.
The scope of this paper covers our observations on the Prediction Task \textit{only}.


}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Analysis: Participants' Cognitive Styles
\draftStatus{D1.8}
}

\boldify{Similar to other works, we used participants' responses to the GenderMag cognitive style survey to classify, along each spectrum, where people fell relative to the median of the distribution.}

We analyzed the data using participants' information processing responses to the GenderMag cognitive style survey. 
The GenderMag survey uses 9-point Likert questions to gather respondents' self-reported cognitive styles for the GenderMag facets, relative to the respondents' peers.
Three of the survey's questions focus on information processing style: 
\textit{I want to get things right the first time, so before I decide how to take action, I gather as much information as I can;
I always do extensive research and comparison shopping before making important purchases;} 
and
\textit{When a decision needs to be made, it is important to me to gather relevant details before deciding, in order to be sure of the direction we are heading.}
Since these questions are intended as relative measurements relative to respondents' peer group, we follow the common practice~\cite{guizani2022debug,anderson-diversity-2022,vorvoreanu2019gender} of defining the peer group to be the other participants in the experiment. 
%to gauge their position on each of the spectra, relative to their peers in the \textit{same treatment}. %MMB: commented out because I think we changed away from "same treatment"
For example, if the sum of a participants' responses for the set of questions about information processing style was above the median, they were considered as having a more comprehensive information processing style than their peers.
It is a validated questionnaire~\cite{guizani2022debug}, and has been used by several studies in the research literature~\cite{guizani2022debug,vorvoreanu2019gender,anderson-diversity-2022}.
% \FIXED{MMB: if accepted, replace the validated questionnaire ref to the (Hamid et al. 2023) book chapter ref (if it is also accepted)}



%----------------------------------
\subsection{The Explainees Processing the Information 
\draftStatus{D2}
}

\boldify{Turning to foundations, we need....}

For human explainees, understanding an AI system through its explanations is a problem-solving activity.
Thus, understanding how these humans work their way through such an activity requires turning to foundations on how people problem solve and gather information.
Also, the foundations need to be relevant to problem-solving in XAI contexts, and fine-grained enough to account for in-the-moment puzzlements that arise when problem-solving with XAI.
Finally, for credibility, the style needs to be reliably measurable, which usually means using a validated questionnaire.

\boldify{here is the competition: NFC, IFT}

One possible foundation is Need for Cognition (NFC).
NFC is the extent to which someone enjoys activities requiring cognitive effort~\cite{cacioppo1982needForCognition,petty2009needForCognition,wu2014needCognition+InfoScent}.
Although NFC fulfills the criteria, it measures something a little different from  how much information people gather and when they gather it; rather, it is more about whether they \emph{enjoy} a variety of cognitively effortful activities.
Another possible foundation is Information Foraging Theory (IFT)~\cite{pirolli1995IFT, pirolli2003snifAct}.
Researchers have employed IFT to understand how people gather information in technology spaces (e.g.,~\cite{piorkowski2016foragingFundamentally, kuttal2019endUserIFT, srinivasa2016foraging, schnabel2019IFTrecommenders}).
However, IFT is reactive to details in the environment; in fact, its low level may be why there appears to be no survey that tries to gather individual IFT ``styles.''

\boldify{GM's info proc fulfills these criteria, and we chose it.
GenderMag is a method that detects inclusivity biases.}

The GenderMag's information processing style also fulfills these criteria, and is the foundation we chose for our investigation.
GenderMag is a method to enable software professionals to systematically locate gender-inclusivity ``bugs'' in the user-facing portions of their software.
It is in reasonably wide use by technologists to understand how to support their diverse users, and has been applied to a variety of domains, including: software/webware for educational settings (e.g.,~\cite{burnett2016gendermag-jrnl,chatterjee2022inclusivity, shekhar2018genderMagLearningSystem, hilderbrand2020genderMagTalesTrenches, lee2014gidget-CSEd}), mobile apps (e.g.,~\cite{burnett2016finding-chi}), digital libraries (e.g.,~\cite{cunningham2016supporting}), software tools/environments,~\cite{padala2020gender,gralha2019genderMagExperiment,mendez2018openSource, guizani2022debug}) and---most pertinent to this paper---AI-oriented systems (e.g.,~\cite{anderson-diversity-2022, burnett2016finding-chi, showkat2018genderMagTelerobotics,vorvoreanu2019gender}).


\boldify{GM has 5 facets; the facet we care about in this paper is Info Processing}

At the core of the GenderMag method are five cognitive styles, or \textit{facets}, each backed by extensive foundational research~\cite{burnett2016gendermag-jrnl, stumpf2020gender}.
The facet we used is the Information Processing facet.
Although the information processing facet has some overlap with NFC, its strength is that it describes/predicts how much and how often a user gathers new information to make decisions about actions to take.
Comprehensive information processors gather information comprehensively---that is, by gathering large batches of information before acting upon what they found.
At the opposite end of the information processing spectrum is the selective information processor, who prefers to gather tiny bits of information, act upon the first promising information they find, then gather a little more and act a little more, course-correcting and gathering more as needed~\cite{meyers2015revisiting, burnett2016gendermag-jrnl, stumpf2020gender}.

We have found other works that explicitly gather participants' information processing styles to analyze participants' user experiences with an AI system.
Anderson et al.~\cite{anderson-diversity-2022} gathered participants' GenderMag cognitive styles and analyzed participant attitudes toward certain AI products (presented via vignettes) according to these styles.
The results showed differences in participants' attitudes depending on their cognitive styles.
Their analysis focused primarily on the \emph{risk} cognitive style, whereas this paper focuses on \emph{information processing style}.
A closely related work is the Riefle et al.~\cite{riefle2022influence}
study on how users with rational and intuitive thinking cognitive styles (participants had to each have a Bachelors degree) understand different types of AI explanations.
They approach understanding of explanations as a decision-making activity and focus on opaque (post-hoc) explanation types: feature-importance, rule-based, and example-based explanations.
Results showed that in regards to their understanding of the explanations, rational participants assessed feature-importance explanations most positively while intuitive participants had the same view of example-based explanations.
All participants performed the best with example-based explanations when their understanding was tested with problem-solving tasks.
How did all these participants differently use these explanations in the problem solving tasks? Our work complements their study by interrogating how diverse cognitively-styled people understand a particular AI system using AI explanations.
We  are interested in how people differ in their use of explanations to problem-solve AI tasks.



%-----------------------------------------------------------
%Ancient leftovers follow...

%\boldify{MMB: these are leftover words. I don't think we need them, but if so don't know where they go.}
%Users usually develop different mental models even for the same AI system e.g. robots so, for accurate predictions, the robot should \emph{``adapt to the particulars''} of the user~\cite{dragan2013legibility}.
%Effective human-AI interactions require that the AI system communicates its intent clearly and that the human understands this intent such that they can accurately predict the AI system's next move. 


%\boldify{MMB: these are leftover words, probably were trying to sunset this subsec. But they're not needed; above parag ends better than this. cutting them.}
%Consideration of human characteristics improve the human-AI collaboration.
%We further the research works described previously by examining the effects of information processing style, a human problem-solving cognitive style, on predictions in a human-AI environment with AI explanations.  
